Learning by stochastic serializations

Complex structures are typical in machine learning. Tailoring learning algorithms for every structure requires an effort that may be saved by defining a generic learning procedure adaptive to any complex structure. In this paper, we propose to map any complex structure onto a generic form, called serialization, over which we can apply any sequence-based density estimator. We then show how to transfer the learned density back onto the space of original structures. To expose the learning procedure to the structural particularities of the original structures, we take care that the serializations reflect accurately the structures' properties. Enumerating all serializations is infeasible. We propose an effective way to sample representative serializations from the complete set of serializations which preserves the statistics of the complete set. Our method is competitive or better than state of the art learning algorithms that have been specifically designed for given structures. In addition, since the serialization involves sampling from a combinatorial process it provides considerable protection from overfitting, which we clearly demonstrate on a number of experiments.

==> Gnuplot/Likelihood_Plot/gnuscript <==
set terminal pdfcairo enhanced
set key left top
set output "out.pdf"
set pointsize 0.3
set xlabel "Number of Iterations"
set ylabel "-ln(P(y|x))"
set xrange [0:30000]
plot  \
1/0 ls 7 lw 6 lc rgb "blue" title "RNN", \
1/0 ls 7 lw 6 lc rgb "red" title "S-RNN", \
1/0 ls 7 lw 6 lc rgb "gray" title "S-RNN {/Symbol l}=100", \
1/0 ls 7 lw 6 lc rgb "green" title "S-RNN {/Symbol l}=10000", \
'rnn' using 1:2 with points pt 7 lc rgb "blue" notitle  , \
'mine' using 1:2 with points pt 7 lc rgb "red" notitle , \
'mine_wc_100' using 1:2 with points pt 7 lc rgb "gray" notitle , \
'mine_wc_10000' using 1:2 with points pt 7 lc rgb "green" notitle , \


==> Gnuplot/Likelihood_Plot/gnuscript2 <==
set terminal pdfcairo
set key left top
set output "out.pdf"
set pointsize 0.3
set xlabel "Number of Iterations"
set ylabel "-ln(P(y|x))"
plot  \
1/0 ls 7 lw 6 lc rgb "black" title "training", \
1/0 ls 7 lw 6 lc rgb "green" title "testing", \
'out_join' using 2:3 with points pt 7 lc rgb "black" notitle  , \
'rnn' using 1:2 with points pt 7 lc rgb "green" notitle  , \


==> Gnuplot/Likelihood_Plot/gnuscript3 <==
set terminal pdfcairo
set key left top
set output "out.pdf"
set pointsize 0.3
set xlabel "Number of Iterations"
set ylabel "-ln(P(y|x))"
set xrange [0:30000]
plot  \
1/0 ls 7 lw 6 lc rgb "black" title "training", \
1/0 ls 7 lw 6 lc rgb "green" title "testing", \
'out_join_mine' using 2:3 with points pt 7 lc rgb "black" notitle  , \
'mine' using 1:2 with points pt 7 lc rgb "green" notitle  , \


==> Gnuplot/Likelihood_Plot/gnuscript_back <==
set terminal pdfcairo
set key left top
set output "out.pdf"
set pointsize 0.001
set xlabel "Number of Iterations"
set ylabel "-ln(P(y|x))"
set xrange [0:30000]
plot  \
1/0 ls 7 lw 6 lc rgb "blue" title "RNN", \
1/0 ls 7 lw 6 lc rgb "black" title "Discriminative RandomRNN", \
1/0 ls 7 lw 6 lc rgb "red" title "Generative RandomRNN", \
1/0 ls 7 lw 6 lc rgb "gray" title "Generative RandomRNN WC 100", \
1/0 ls 7 lw 6 lc rgb "green" title "Generative RandomRNN WC 10000", \
'rnn' using 1:2 with dots pt 7 lc rgb "blue" notitle  , \
'e-rnn' using 1:2 with dots pt 7 lc rgb "black" notitle , \
'mine' using 1:2 with dots pt 7 lc rgb "red" notitle , \
'mine_wc_100' using 1:2 with dots pt 7 lc rgb "gray" notitle , \
'mine_wc_10000' using 1:2 with dots pt 7 lc rgb "green" notitle , \


==> Gnuplot/Likelihood_Plot/gnuscript_long <==
set terminal pdfcairo
set key left top
set output "out.pdf"
set pointsize 0.3
set xlabel "Number of Iterations"
set ylabel "-ln(P(y|x))"
#set xrange [0:30000]
plot  \
1/0 ls 7 lw 6 lc rgb "blue" title "RNN", \
1/0 ls 7 lw 6 lc rgb "red" title "StructRNN", \
1/0 ls 7 lw 6 lc rgb "gray" title "StructRNN 100", \
1/0 ls 7 lw 6 lc rgb "green" title "StructRNN 10000", \
'rnn' using 1:2 with points pt 7 lc rgb "blue" notitle  , \
'mine' using 1:2 with points pt 7 lc rgb "red" notitle , \
'mine_wc_100' using 1:2 with points pt 7 lc rgb "gray" notitle , \
'mine_wc_10000' using 1:2 with points pt 7 lc rgb "green" notitle , \


==> Gnuplot/Likelihood_Plot/gnuscript_new <==
set terminal pdfcairo
set key left top
set output "out.pdf"
set pointsize 0.3
set xlabel "Number of Iterations"
set ylabel "-ln(P(y|x))"
set xrange [0:30000]
set yrange [-150:500]
plot  \
1/0 ls 7 lw 6 lc rgb "blue" title "RNN testing", \
1/0 ls 7 lw 6 lc rgb "red" title "StructRNN testing", \
1/0 ls 7 lw 6 lc rgb "black" title "RNN training", \
1/0 ls 7 lw 6 lc rgb "green" title "StructRNN training", \
'rnn' using 1:2 with points pt 7 lc rgb "blue" notitle  , \
'out_join' using 2:3 with points pt 7 lc rgb "black" notitle  , \
'out_join_mine' using 2:3 with points pt 7 lc rgb "green" notitle  , \
'mine' using 1:2 with points pt 7 lc rgb "red" notitle , \


==> Gnuplot/like_comp/gnuscript <==
set terminal pdfcairo
set key left top
set output "out.pdf"
set pointsize 0.1
set xlabel "NB Gradient update"
set ylabel "-ln(P(a))"

#set xrange [0:4000]
plot  \
1/0 ls 7 lw 6 lc rgb "blue" title "StructRNN Train", \
1/0 ls 7 lw 6 lc rgb "red" title "StructRNN Test", \
'out_join' using 2:3 with points lc rgb "blue" notitle  , \
'out_join' using 2:5 with points lc rgb "red" notitle , \


==> Propositional-short.tex <==
\paragraph{Propositional datasets}
\label{sec:propositional-short}
Here we experiment on a set of standard classification datasets taken from UCI. 
We serialise a vectorial instance as a sequence which we generate by randomly sampling features without replacement. We compare 
against a Multi Layer Perceptron (MLP) which has an equivalent architecture to our \strucLearn model. As before a detailed description 
of the experiments and the results can be found in the respective section (\ref{sec:propositional}) of the appendix. The accuracy 
of the two methods is very similar over all the datasets (see appendix, table \ref{tab:prop}). However what is striking is the 
resistance to overfitting that \strucLearn exhibits with respect to the length of training when compared to the standard MLP.
With the exception of the iris dataset, which probably due to its small number of features that does not allow 
for the randomization effect to kick in, the loss values in the training/validation/test sets are very similar
for \strucLearn, i.e. there is hardly any divergence. MLP, in all datasets except iris exhibits considerable
divergence between the different losses, which takes place rather early in the learning. These empirical results confirm what we 
already observed in the previous data structures, i.e. that the randomization inherent in the serialisation process brings a robust 
protection against overfitting, allowing training to continue for considerably longer horizons.


==> Propositional.tex <==
\subsection{Propositional datasets}
\label{sec:propositional}
We also explore the performance of \strucLearn on a set of standard propositional classification datasets taken from the UCI repository.
These datasets have a mix of $d_n$ numeric and $d_c$ categorical attributes. Given a training instance $\mathbf x$ 
we will use $\mathbf x^{d_n} \in \mathbb R^{d_n}$ to denote the vector of its numerical components 
and $\mathbf x^{d_c} \in \mathbb N^{d_c}$ to denote the vector of its categorical components.  We denote by $y$ the
label of $\mathbf x$, and $y \in \mathbb Y=\{1,\ldots ,c\}$. We use \strucLearn to learn the joint probability 
 $\Pr(\mathbf x,y)$ which we use to classify instances according to the $\argmax_{y}\Pr(y|\mathbf x)$ 
 rule. We evaluate the performance using predictive accuracy. 

\subsubsection{Serialisation of propositional instances}
We now describe the serialisation structure that the \strucAlgo produces for a particular 
learning instance ($\mathbf x, y$). Our dictionary $\mathbb B$ contains real-valued and categorical
elements. The domain of the categorical elements is the set of the feature names together with the 
set of values of all the categorical attributes. Thus 
$\mathbb B=\{l(x^{d_n}_i)|i := 1...d_n\} \cup \{l(x^{d_c}_i)| i := 1...d_c\} \cup l(y) \cup \mathbb Y \cup \mathbb R$.
One should pay attention that every feature name and value of discrete features have a unique name.
As before $l(x_i)$ is a function which returns the name $x_i$ feature. 
Within a serialisation a numerical feature name is always coupled by its respective value, while a categorical 
feature name is always coupled with zero. The categorical elements of the dictionary are
encoded as one-hot vectors. To serialise an instance the serialiser selects randomly,
among its features that are not yet included in its serialisation, the next one for inclusion. 
To describe the state $s$ of a partial serialisation of learning instance $(\mathbf x, y)$ we use the set 
of $(l(x_i), x_i), (l(y),y)$, i.e. feature names and their values, that have been so far included in the 
serialisation. It is easy to check equality between partial serializations in order to use it within the structural 
constraint regulariser, by checking a set equality over the respective state representations. 
\note[Alexandros-NIPS]{Have we done the same discussion on all the other data types?}

\subsubsection{Learning architectures for propositional instances}
We compare \strucLearn against a standard Multilayer Neural Network baseline trained 
using the cross entropy loss. We tune the architecture of the baseline by doing a grid search to select 
the number of layers from (1,2,3) and the number of hidden units from (32,64,128,256). For \strucLearn 
we use the same learning architecture as the one described in \ref{sec:dynamical-system} with small modifications 
in the number of layers and hidden units. We use a two-layer and 256 unit LSTM and we use the same range of values
as our baseline to determine the number of the hidden units for the neural-network that computes the mean, 
covariance matrix and mixture components. The regularisation parameter $\lambda$ is selected from (0,1,10,100). 
The number of mixture components is 6. We train with early stopping on the validation set. We evaluate
the predictive accuracy on a hold-out test set whenever this is available (images, pendigits); 
if a hold-out test set is not available then we use one third of the instances as hold out. The 
validation set is one sixth of the total instance number when no hold-out set was given; when a 
hold-out set is given you remove one quarter and use it for validation set. The detailed training
and testing sizes, together with a short description of the datasets is given in table~\ref{tab:prop}.
\note[Alexandros-NIPS]{Completely senseless/incoherent procedure to create train/test/validation sets.}
As before we use ADAM to optimize, with a mini batch 
of size 32 for the baseline, and a mini batch size of 64 instances generated 
from 32 real instances by generating two serialisations for each one of them for \strucLearn.

\subsubsection{Results for propositional problems}
We give the evaluation results in table \ref{tab:prop}. \strucLearn has a performance that is similar to 
the MLP baseline. The reason is that for such simple tasks our model does not have any additional information 
that it can use, compared to the information available to the standard baseline. 

Once again we remark the resistance of \strucLearn to overfitting. We give in figure \ref{fig:figurelossimage} the evolution of 
the log-likelihood and the cross-entropy loss on the training/validation/test sets for \strucLearn and the MLP baseline, respectively, 
for all propositional datasets. We rescaled the $y$-axis into [0,1] for both losses for comparability. 
As we can see, the divergence of the three losses for the \strucLearn is very small (with the exception of iris), 
even after 6000 training iterations. In fact in the German and pendigits datasets we never observed a divergence
up to the 10k training iterations that we let \strucLearn run for. We believe that the overfitting protection does 
not kick-in for iris due to the very small number of features (only four) which means that there is not enough
diversity in the generated serialisations; a set of 4 features has only 24 reorderings. On the other hand the 
MLP baseline shows large to very large divergences between the training/validation/test set losses, and this 
rather early in the training iterations (2k training steps or even earlier). 

\note[Alexandros-NIPS]{Nice figure, but what happens with the baseline? maybe it does not overfit either?}

\begin{table}
\begin{tabular}{ccccccc}
	Dataset & \# Training instances& \# Testing instances & \#features & \#Classes & \strucLearn & MLP \\
	\hline
	German&686&250&20&2&75\%&78\%\\
	Image&210&2038&19&7&93\%&88\%\\
	Iris &75&50&4&3&99\%&99\%\\
	Pendigits&7494&3498&16&10&89\%&89\%\\ \hline
\end{tabular}
\caption{Predictive accuracy for the propositional classification datasets.}
\label{tab:prop}
\end{table}

\begin{figure}[htbp]
	\centering
	Image\\
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/Image/figure_Loss_Image}
		\centering\strucLearn
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
	\includegraphics[width=\linewidth]{Gnuplot/Image/Loss_Baseline}
	\centering MLP
\end{minipage}

	\centering
	German\\
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/German/german_mine.pdf}
		\centering\strucLearn
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/German/german_nn.pdf}
		\centering MLP
	\end{minipage}

	\centering
	Pendigits\\
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/pendigits/pendigits_mine.pdf}
		\centering\strucLearn
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/pendigits/pendigits_nn.pdf}
		\centering MLP
	\end{minipage}

	\centering
	Iris\\
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/iris/iris_mine.pdf}
		\centering\strucLearn
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\includegraphics[width=\linewidth]{Gnuplot/iris/iris_nn.pdf}
		\centering MLP
	\end{minipage}
	\caption{Evolution of the conditional negative log-likelihood loss and cross-entropy in training/validation/test sets 
	as a function of the training iterations for \strucLearn (left) and the MLP baseline (right) respectively.}
	\label{fig:figurelossimage}
\end{figure}


==> mapping_with.tex <==
\note[Removed]{\subsection{Serialization with structural constraints}
\label{Serializer} }
\note[Steph]{Section heading to be removed I think}
\note[Alexandros]{Yes, moved to previous section.}

\note[Removed]{Let us now look how the work we have done in section \ref{Manifold} need to be adapted for the case when we have probabilistic constraints.
Obtaining the probability on the original space given the probability in the transformed space does not change, however the algorithm \ref{alg:SamplingEasy} need to be modified to ensure that the sampling strategy we use to sample $a\in \mathbb{A}$ does respect equation \ref{Prob:state}. Imposing the constraints make the algorithm more complicated because theses equations imposes correlations between different instances that share the same subsequence, this force us to work at the same time at the element by element level and the full sequence level.
For this case, we redefine the function $\mu$ to give a weight on the element level by defining it as $\mu: \mathbb{S}\times \mathbb{B} \mapsto \mathbb{R}_{>0}$.
As before algorithm \ref{alg:Sampling} tell us for every $x\in \mathbb{X}$ how to obtain samples in the $a\in\mathbb{A}$ space together with $\Pr(O=o|X=x)$ needed to use equation \ref{FracProb}. The main change of algorithm \ref{alg:Sampling} with respect to \ref{alg:SamplingEasy} is the sampling of $a\in\mathbb{A}$ instead of being directly sampled, we iteratively construct the sample $a$ by sampling the next possible element. This allows us to compute the state in parallel to the sampling of the next element, ensuring that the constraints of equation \ref{Prob:state} are respected because the weight function $\mu$ depend on the state.
}

\note[Removed]{Modeling with states enables the expression of structural constraints on the serializations.
These constraints create correlation between (sub-)serializations and prevent us to sample serializations at once, as described earlier.
Instead, we adapt our sampling measure $\mu$ to reflects the constraints within the sequences and therefore sample at the level of the serialization element.
In other words, we adapt $\mu$ to express how the next element $a^{t+1}$ is sampled from $\mathbb B$ with respect to the state $s^t\in\mathbb S$.
We redefine the measure $\mu$ as $\mu: \mathbb{S}\times \mathbb{B} \rightarrow \mathbb{R}_{>0}$ to provide a measure over the joint set of states ($s^t$) and the lexicon from where $a^{t+1}$ will be sampled.
Algorithm \ref{alg:Sampling} then describes the adapted serialization procedure with constraints.
Given $x$, a serialization is obtained by sampling at each time step a new ``next element'' $a^{t+1}$ from the set of all plausible such elements, constructed from inspecting $X^{-1}(x)$ a timestep $t+1$, according to the state $s^t$ and $\mu$.
}
\note[Alexandros]{Pushed to previous section}

\note[Steph]{@Pablo: In practice, are you actually using $\mu$ and if yes how do you define it? Or is it just abstract talk and actually you just randomize the next element wrt constraints algorithmically? ie do you really follow Algo 2???}
\note[Steph]{@Pablo: In fact the exact same questions go for $f$ in Algo 2. Is it an abstract statement? Or how do you define $f$?}
\note[Steph]{@Pablo: Why $O$ is an input parameter in Algo 1 and 2??}

\note[Removed]{The training procedure is the same than for section \ref{Manifold} by replacing algorithm \ref{alg:SamplingEasy} by \ref{alg:Sampling}. The learner minimize:
\begin{equation}\label{MaxLikelihood}
\tilde{\Pr}(A)=\argmin_{\tilde{\Pr}(A)}  \KL(\hat{\Pr}(A)||\tilde{\Pr}{A})
\end{equation}
By construction $\hat{\Pr}(A)\in \mathcal{M}$ because it respect equation \ref{Prob:state} which also mean that for a strong enough model we would expect that the same is true for $\tilde{\Pr}(A)$ however we cannot prove it because we lack a result similar to the triangular inequality for KL divergence.
}
\note[Steph]{Useless since it repeats the objective function as before}


==> overview.tex <==
\subsection{Overview}

We model the data distribution by disentangling two related concepts,the learning of the data distribution and the modelling of the data structure. This disentanglement is carried out by mapping the original data into a stochastic process whose realisations are sequences of elementary components (scalars, vectors).
We will call theses multiple sequences \emph{serialisations}.
Computing multiple realisations of the stochastic process for every original data instance creates a dataset on which we train a generic sequence density estimator model like an RNN \citep{GravesSequence}.
The use of a standard sequences density estimator enable the use of the recent improvement like LSTM \citep{LSTM}, NTM \citep{NTM} and DNC \citep{graves_hybrid_2016} without any changes. We will, for the rest of the paper describe the framework for an RNN.
The description of the new space can be found in section \ref{newSpace} and the description of the mapping in section \ref{Manifold}.

However, by completely disentangling the learning algorithm from the data structure, we loose all the domain knowledge and properties of the data which is fundamental in learning.
To preserve this information, we define an interface which enable the expression of the domain knowledge and inherent properties of the data in a generic way which can be used by the learning algorithm even without knowing the nature of the data. The key information about the structure is based on the factorisation of the conditionals. We express this factorization with the help of the notion of state which represents the relevant information that the system has acquired after a given step of the sequence about the following steps. The inherent properties of the structure is expressed by the transitions between states as a new elementary component is received, for example invariance of ordering is expressed by the fact that following two different orders (of elementary component) leads to the same state.
The detailed description of the state is found in section \ref{ProbStructure}.
% The representation used for the state is domain specific and allows to incorporate information about the inherent properties of the data.

%TODO move into section 2
This state representation is used in two ways. First to ensure that the empirical distributions of the serialisations generated from the original training instances are consistent with the inherent properties of the structure.
For example, for an order invariant data structure the probability of the following elements of the sequences does not depend on the order of previous elements thus ensuring that the data used to train the sequence generator model does not contain wrong inherent properties.
Doing this will indirectly ensure that the hidden states of two different serialisations of the same instance are equivalent\footnote{We consider that two hidden states are equivalent if the output of the network using either values of the hidden states is the same, i.e. there is no observable effect when changing the hidden state.} because the target of both networks are the same. This is similar to what is done in orderless NADE \citep{NadeUriaCGML16} to impose order invariance for vector density estimation however done on more complex structures. Detailed description is found in section \ref{Serializer}.

Second, we propose a regularized version of our framework for RNN like algorithm which in addition to the serialisation provides the information which hidden state should be the same.
This constraint was used in TwinNet \citep{twinnet} to enforce the consistency  for the specific data structure of sequence data given in the forward order and backward order. Imposing constraints on the hidden state of an RNN transforms the linear structure of the RNN into a general graph structure.
This will be describes in details in section \ref{Regularizer}.


==> regularizer.tex <==
\subsection{Regularized learning}
\label{Regularizer}
Having constructed a valid training set $\mathcal A$ transferring our domain knowledge onto $\mathbb A$, we use a RNN to learn $P_{\mathbb A,\vect \phi}$.
We can support the RNN in its learning by way of a regularizer constructed around the constraints of our domain.
To this end, we use equation \ref{equivalencestate} again and create a binary sparse matrix $\left(C_{jk}^t\right)$ (${j,k=1\dots|\mathcal A|}, {t=1\dots T}$) storing state equivalences with the serializations $a_j\in \mathcal A$ (ie $C_{jk}^{t}=1$ iff $s_{j}^t=s_{k}^{t}$).
%% \begin{equation}
%%   C_{jk}^{t}=
%%   \begin{cases}
%%     1& \text{If } s_{j}^t=s_{k}^{t}\\
%%     0& \text{0therwise}
%%   \end{cases}
%% \end{equation}
%% Ones in the constraint matrix indicate that the past information of the two states are the same which forces the probability of the next element to have:
%% \begin{equation}\label{equivalence2}
%% \Pr(A|s^t_{i})=\Pr(A|s^{t'}_{i'})
%% \end{equation}

%% The solution for the probability distribution if the density estimator uses maximum likelihood is modified from equation \ref{MaxLikelihood} to:
%% \begin{align}
%% \tilde{\Pr}(A)&=\argmin_{\tilde{\Pr}(A)}  \KL(\tilde{\Pr}(A)||\hat{\Pr}(A))
%% \intertext{Subject to}
%% \tilde{\Pr}(X=x)&\in\mathcal{M} \quad \forall x\in \mathcal{X}
%% \end{align}
%% Where the constraint mean that our model respect the structure of the data and probabilistic assumptions on the training data.

%Let define $\bbespilon$ a noise space and $\epsilon\in \bbespilon$. Let define the serialisation strategy function $\Gamma:\bbespilon\times \mathbb{D}\mapsto \tau$ which given the noise and data give a serialisation. Ideally, we would sample iid sample from $\Pr(D)$ and $\Pr(\epsilon)$ and obtain iid sample from $\Gamma(\epsilon,D)$ which is described by the probability:
%\begin{equation}
%\label{SampleDistrib}
%\Pr(\Gamma(\epsilon,D))=\sum_{\epsilon'}\Pr(D)\Pr(\epsilon')\mathbbm{1}(\Gamma(\epsilon',D)-\Gamma(\epsilon,D))=\Pr(D)\underbrace{\sum_{\epsilon'}\Pr(\epsilon')\mathbbm{1}(\Gamma(\epsilon',D)-\Gamma(\epsilon,D))}_{p}
%\end{equation}
%Where we have used the fact that every serialisation come from a single data instance however multiple noise parameter can give the same serialisation and that the noise and the data are independent. The sequences that the density estimator receive are iid sample of probability given by equation \ref{SampleDistrib} related by a known transformation to the probability of the original data. This mean that if the density estimator correctly does its work in training a density estimator in the space of serialisation we recover the correct probability distribution in the original data space.
%
%To force the model to learn a probability distribution from the statistical manifold we want to ensure that the data we serialize could come from an unknown distribution from the statistical manifold.


==> sampling.tex <==
\subsection{Sampling in the original data space:}

To sample from the original data space, we first sample in the transformed space using the learned model obtaining a sequence $a\in \mathbb{A}$. The final result is given by using the random variable $X$ by:
\begin{equation}
x=X(a)
\end{equation}
